Attention and Anticipation in Fast Visual-Inertial Navigation

We study a Visual-Inertial Navigation (VIN) problem in which a robot needs to estimate its state using an on-board camera and an inertial sensor, without any prior knowledge of the external environment. We consider the case in which the robot can allocate limited resources to VIN, due to tight computational constraints. Therefore, we answer the following question: under limited resources, what are the most relevant visual cues to maximize the performance of visual-inertial navigation? Our approach has four key ingredients. First, it is task-driven, in that the selection of the visual cues is guided by a metric quantifying the VIN performance. Second, it exploits the notion of anticipation, since it uses a simplified model for forward-simulation of robot dynamics, predicting the utility of a set of visual cues over a future time horizon. Third, it is efficient and easy to implement, since it leads to a greedy algorithm for the selection of the most relevant visual cues. Fourth, it provides formal performance guarantees: we leverage submodularity to prove that the greedy selection cannot be far from the optimal (combinatorial) selection. Simulations and real experiments on agile drones show that our approach ensures state-of-the-art VIN performance while maintaining a lean processing time. In the easy scenarios, our approach outperforms appearance-based feature selection in terms of localization errors. In the most challenging scenarios, it enables accurate visual-inertial navigation while appearance-based feature selection fails to track robot's motion during aggressive maneuvers.

==> extensions.tex <==
%!TEX root = main.tex

\section{Extensions}
\label{sec:extensions}

\LC{Considerations on notation: $\Deltaij$ is inconsistent, $k$ and $j$ might not be the best choice of time stamps}

- requirement matrix that multiplies the covariance/ info matrix (diagonal)
- select minimum number of features such that metric is below a bound

- select k features to minimize uncertainty
- select min features to bound uncertainty

\myparagraph{Computation}
\LC{faster computation by parallelization and sparse matrix manipulation}

==> imuNonlinearModel.tex <==
%!TEX root = main.tex

\subsubsection{IMU Model}
\label{sec:imuModel}

Our simplified IMU model is based on a single assumption. The accumulation of the rotation error due to gyroscope 
integration over the time horizon is negligible. In other words, the relative rotation estimates predicted by the 
gyroscope are accurate. This assumption is realistic, even in inexpensive commercial IMUs: in the experimental 
section we show that rotation errors from gyroscope  are negligible when integrating over tens of seconds, 
which is way being what we need here (a typical horizon in our attention system if $\hor = 3$s). 

Assuming that the rotations are accurately known allows restricting the state to the robot position, linear velocity, 
and the accelerometer bias. Therefore, in the rest of this paper, the state of the robot at time $k$ is 
  $\vxx_k \doteq [\pos{k} \; \vel{k} \; \biasA{k} ]$, where $\pos{k} \in \Real{3}$ is the 3D position of the 
  robot at time $k$, $\vel{k} \in \Real{3}$ is its velocity, and $\biasA{k}$ is the (time-varying) accelerometer bias.
  We also use the symbol $\Rot{k}$ to denote the attitude of the robot at time $k$: this is assumed to be known from 
  gyroscope integration over the 
  horizon $\hor$, hence it is not part of the state.

An IMU commonly includes a 3-axis accelerometer and a 3-axis gyroscope and allows measuring the rotation rate and the acceleration of the sensor with respect to an inertial frame. 
The measurements, namely ${}_\imu\tilde\acc(t)$, and ${}_\imu\tilde\rotvel_{\world\imu}(t)$, are affected by additive white noise $\noise$ and a slowly varying sensor bias $\bias$:
%
\bea
  {}_\imu\tilde\rotvel_{\world\imu}(t)
    &=& {}_\imu\rotvel_{\world\imu}(t) + \bias^g(t) + \noise^{g}(t) \label{eq:omegaModel}\\
  {}_\imu\tilde\acc(t)
    &=& \R_{\world\imu}\tran(t)\left({}_\world\acc(t) - {}_\world\gravity \right) + \bias^a(t) + \noise^{a}(t), \label{eq:accModel}
\eea
In our notation, the prefix $\Imu$ denotes that the corresponding quantity is expressed in the frame $\Imu$.
The pose of the IMU is described by the transformation $\{\R_{\world\imu}, {}_\world\tran\}$, which maps a point from sensor frame $\Imu$ to $\World$.
The vector ${}_\imu\rotvel_{\world\imu}(t) \!\in\! \Real{3}$ is the  instantaneous angular velocity of $\Imu$ relative to $\World$ expressed in coordinate frame $\Imu$, while ${}_\world\acc(t) \!\in\! \Real{3}$ is the acceleration of the sensor; ${}_\world\gravity$ is the gravity vector in world coordinates. We neglect effects due to earth's rotation, which amounts 
to assuming that $\World$ is an inertial frame.

We can write ${}_\world\acc$ and ${}_\imu\rotvel_{\world\imu}$ as a function of the IMU measurements:
%
\bea
\label{eq:integration}
  \R(k+1) &=& \R(k)  \expmap{ \left(\tilde\rotvel(t) - \bias^g(t)-\noise^{gd}(t) \right) \Deltak } \nonumber\\
  \V(k+1) &=& \V(k) + \gravity\Deltak + \R(k) \left( \accshort \right) \Deltak \nonumber\\
  \P(k+1) &=& \P(k) + \V(k) \Deltak + \frac{1}{2}\gravity\Deltak^2 + \nonumber \\
  && \frac{1}{2}\R(k) \left( \accshort \right) \Deltak^2,
\eea
%
where we dropped the coordinate frame subscripts for readability (the notation should be unambiguous from now on).

Dropping the rotation part and integrating from time $i$ to time $j$ (keyframe times):
also: assuming constant bias over the interval:
%
\bea
\label{eq:integrationKeyframes}
  \V(j) &=& \V(i) + \gravity\Deltaij + \sum_{k=i}^{j-1} \R(k) \left( \accshortConstBias \right) \Deltak \nonumber\\
  \P(j) &=& \P(i) + \sum_{k=i}^{j-1}  \V(k) \Deltak + \frac{1}{2}\gravity\Deltak^2 + \nonumber \\
  && \frac{1}{2}\R(k) \left( \accshortConstBias \right) \Deltak^2,
\eea
%
where $\Deltaij \doteq  \sum_{k=i}^{j-1} \Deltak$.

Now we define the noise vector and matrices:
%
\bea
\label{eq:definitionsV}
\deltaVmeas\ij = \gravity\Deltaij + \sum_{k=i}^{j-1} \R(k) \tilde\acc(\disctime) \Deltak 
\nonumber \\
\noiseAccd\ij \doteq [\noiseAccd(i)\tran \; \noiseAccd(i+1)\tran \; \ldots \; \noiseAccd(j-1)\tran]\tran
\nonumber \\
J^v\ij = [\R(1)\tran \Delta_1 \;\; \R(2)\tran \Delta_2 \;\; \ldots \;\; \R(j-1)\tran \Delta_{j-1}]\tran
\nonumber \\
\Theta^v\ij = (\sum_{k=i}^{j-1} \R(k) \Deltak)
\eea
%
% \tilde\acc(\disctime)\!-\! \bias^a(i) \!-\! \noiseAccd(\disctime)
Then the expression of $\V(j)$ becomes:
%
\bea
\label{eq:linearMeasurementsV}
 \deltaVmeas\ij &=& \V(j) - \V(i) + \Theta^v\ij \bias^a(i)  + J^v\ij \noiseAccd\ij
\eea
%
Similarly, we can develop the expression of $\P(j)$ as follows:
%
\bea
\label{eq:definitionsP}
\deltaPmeas\ij = \sum_{k=i}^{j-1} \Deltak \deltaVmeas\ik + \half ( \gravity + \R(k) \tilde\acc(\disctime) ) \Deltak^2 
\nonumber \\
J^p\ij = [\R(1)\tran \Delta_1 \;\; \R(2)\tran \Delta_2 \;\; \ldots \;\; \R(j-1)\tran \Delta_{j-1}]\tran
\nonumber \\
J^p\ij = \sum_{k=i}^{j-1}  J^v\ik \Deltak + \half[\R(1)\tran \Delta_1^2 \;\; \ldots \;\; \R(j-1)\tran \Delta_{j-1}^2]\tran
\nonumber \\
\Theta^v\ij = \sum_{k=i}^{j-1}  \Theta^v\ik \Deltak + \R(k) \Deltak^2
\eea
%
Then the expression of $\P(j)$ becomes:
%
\bea
\label{eq:linearMeasurementsP}
 \deltaPmeas\ij &=& \P(j) - \P(i) - \V(i) \Deltaij + \Theta^p\ij \bias^a(i)  + J^p\ij \noiseAccd\ij
\eea
%

==> table50-1B-1D.tex <==
%==================================================================== 
\multirow{3}{*}{MH_01_easy}  &  \quality &  $6.25\e{-3}$  &   \multirow{1}{*}{$0.168$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $5.67\e{-3}$  &   \multirow{2}{*}{$0.25$} &   \multirow{2}{*}{ $0.63$ } \\ 
             &      &  \blue{($-9\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $5.46\e{-3}$  &   \multirow{2}{*}{$0.139$} &   \multirow{2}{*}{ $0.21$ } \\ 
             &      &  \blue{($-13\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_02_easy}  &  \quality &  $8.88\e{-3}$  &   \multirow{1}{*}{$0.502$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $6.11\e{-3}$  &   \multirow{2}{*}{$0.418$} &   \multirow{2}{*}{ $0.73$ } \\ 
             &      &  \blue{($-31\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $6.69\e{-3}$  &   \multirow{2}{*}{$0.36$} &   \multirow{2}{*}{ $0.24$ } \\ 
             &      &  \blue{($-25\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_03_medium}  &  \quality &  $1.59\e{-2}$  &   \multirow{1}{*}{$0.637$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $1.42\e{-2}$  &   \multirow{2}{*}{$0.851$} &   \multirow{2}{*}{ $0.64$ } \\ 
             &      &  \blue{($-11\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $1.58\e{-2}$  &   \multirow{2}{*}{$0.38$} &   \multirow{2}{*}{ $0.22$ } \\ 
             &      &  \blue{($-1\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_04_difficult}  &  \quality &  $3.42\e{-2}$  &   \multirow{1}{*}{$0.476$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $4.19\e{-2}$  &   \multirow{2}{*}{$0.409$} &   \multirow{2}{*}{ $4.03$ } \\ 
             &      &  \red{($23\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $2.98\e{-2}$  &   \multirow{2}{*}{$0.501$} &   \multirow{2}{*}{ $0.20$ } \\ 
             &      &  \blue{($-13\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_05_difficult}  &  \quality &  $1.3\e{-1}$  &   \multirow{1}{*}{$131$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $4.53\e{-2}$  &   \multirow{2}{*}{$0.627$} &   \multirow{2}{*}{ $3.97$ } \\ 
             &      &  \blue{($-65\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $3.03\e{-2}$  &   \multirow{2}{*}{$0.723$} &   \multirow{2}{*}{ $0.23$ } \\ 
             &      &  \blue{($-77\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{V1_01_easy}  &  \quality &  $1.09\e{-2}$  &   \multirow{1}{*}{$0.326$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $1.09\e{-2}$  &   \multirow{2}{*}{$0.401$} &   \multirow{2}{*}{ $0.49$ } \\ 
             &      &  \blue{($-1\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $1.07\e{-2}$  &   \multirow{2}{*}{$0.269$} &   \multirow{2}{*}{ $0.2$ } \\ 
             &      &  \blue{($-2\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{V1_02_medium}  &  \quality &  $1.19\e{-1}$  &   \multirow{1}{*}{$136$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $2.67\e{-2}$  &   \multirow{2}{*}{$0.538$} &   \multirow{2}{*}{ $0.89$ } \\ 
             &      &  \blue{($-78\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $2.39\e{-2}$  &   \multirow{2}{*}{$0.665$} &   \multirow{2}{*}{ $0.28$ } \\ 
             &      &  \blue{($-80\%)$}  &              &            \\ 
\cline{2-5}
\hline


==> table50-1B-1L.tex <==
%==================================================================== 
\multirow{3}{*}{MH_01_easy}  &  \quality &  $6.25\e{-3}$  &   \multirow{1}{*}{$0.168$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $5.67\e{-3}$  &   \multirow{2}{*}{$0.25$} &   \multirow{2}{*}{ $0.63$ } \\ 
             &      &  \blue{($-9\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $5.46\e{-3}$  &   \multirow{2}{*}{$0.139$} &   \multirow{2}{*}{ $0.21$ } \\ 
             &      &  \blue{($-13\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_02_easy}  &  \quality &  $8.88\e{-3}$  &   \multirow{1}{*}{$0.502$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $6.11\e{-3}$  &   \multirow{2}{*}{$0.418$} &   \multirow{2}{*}{ $0.73$ } \\ 
             &      &  \blue{($-31\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $6.69\e{-3}$  &   \multirow{2}{*}{$0.36$} &   \multirow{2}{*}{ $0.24$ } \\ 
             &      &  \blue{($-25\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_03_medium}  &  \quality &  $1.59\e{-2}$  &   \multirow{1}{*}{$0.637$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $1.42\e{-2}$  &   \multirow{2}{*}{$0.851$} &   \multirow{2}{*}{ $0.64$ } \\ 
             &      &  \blue{($-11\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $1.58\e{-2}$  &   \multirow{2}{*}{$0.38$} &   \multirow{2}{*}{ $0.22$ } \\ 
             &      &  \blue{($-1\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_04_difficult}  &  \quality &  $6.34\e{-2}$  &   \multirow{1}{*}{$1.3$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $5.07\e{-2}$  &   \multirow{2}{*}{$1.43$} &   \multirow{2}{*}{ $1.2$ } \\ 
             &      &  \blue{($-20\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $4.7\e{-2}$  &   \multirow{2}{*}{$0.992$} &   \multirow{2}{*}{ $0.36$ } \\ 
             &      &  \blue{($-26\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{MH_05_difficult}  &  \quality &  $6.72\e{-2}$  &   \multirow{1}{*}{$1.29$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $6.01\e{-2}$  &   \multirow{2}{*}{$2.56$} &   \multirow{2}{*}{ $1.2$ } \\ 
             &      &  \blue{($-11\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $2.83\e{-2}$  &   \multirow{2}{*}{$0.846$} &   \multirow{2}{*}{ $0.36$ } \\ 
             &      &  \blue{($-58\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{V1_01_easy}  &  \quality &  $1.09\e{-2}$  &   \multirow{1}{*}{$0.326$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $1.09\e{-2}$  &   \multirow{2}{*}{$0.401$} &   \multirow{2}{*}{ $0.49$ } \\ 
             &      &  \blue{($-1\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $1.07\e{-2}$  &   \multirow{2}{*}{$0.269$} &   \multirow{2}{*}{ $0.2$ } \\ 
             &      &  \blue{($-2\%)$}  &              &            \\ 
\cline{2-5}
\hline
%==================================================================== 
\multirow{3}{*}{V1_02_medium}  &  \quality &  $1.19\e{-1}$  &   \multirow{1}{*}{$136$} &   \multirow{1}{*}{ - } \\ 
\cline{2-5}
              &  \multirow{2}{*}{\minEig} &  $2.67\e{-2}$  &   \multirow{2}{*}{$0.538$} &   \multirow{2}{*}{ $0.89$ } \\ 
             &      &  \blue{($-78\%)$}  &              &            \\ 
\cline{2-5}
              &  \multirow{2}{*}{\logDet} &  $2.39\e{-2}$  &   \multirow{2}{*}{$0.665$} &   \multirow{2}{*}{ $0.28$ } \\ 
             &      &  \blue{($-80\%)$}  &              &            \\ 
\cline{2-5}
\hline


==> tableRealResults.tex <==
%!TEX root = main.tex

\begin{table}[h!]
\centering
\begin{tabular}{ |c||c | c|c|c|c| }
\hline
& \multirow{2}{*}{Approach} & Rel. Tran.    &  Abs. Tran.   & Selection  \\
&   &  Error [\meters]  &   Error [\meters] &  Time [\sec] \\
\hline
\input{table50-1B-1L.tex}
\end{tabular}
\caption{EuRoC datasets results on a 50-feature budget. \label{tab:realResults}}% 
\end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{ |c||c | c|c|c|c| }
% \hline
% & \multirow{2}{*}{Approach} & Rel. Tran.    &  Abs. Tran.   & Selection  \\
% &   &  Error [\meters]  &   Error [\meters] &  Time [\sec] \\
% \hline
% \input{./figures/results/table50-1L.tex}
% \end{tabular}
% \caption{x \label{tab:parameters}}% 
% \end{table}

==> visionModel.tex <==
%!TEX root = main.tex

\subsubsection{Vision Model}
\label{sec:visionModel}
